Approximating the Maximum Independent Set of Convex Polygons with a Bounded Number of Directions

In the maximum independent set of convex polygons problem, we are given a set of $n$ convex polygons in the plane with the objective of selecting a maximum cardinality subset of non-overlapping polygons. Here we study a special case of the problem where the edges of the polygons can take at most $d$ fixed directions. We present an $8d/3$-approximation algorithm for this problem running in time $O((nd)^{O(d4^d)})$. The previous-best polynomial-time approximation (for constant $d$) was a classical $n^\varepsilon$ approximation by Fox and Pach [SODA'11] that has recently been improved to a $OPT^{\varepsilon}$-approximation algorithm by Cslovjecsek, Pilipczuk and W\k{e}grzycki [SODA '24], which also extends to an arbitrary set of convex polygons. Our result builds on, and generalizes the recent constant factor approximation algorithms for the maximum independent set of axis-parallel rectangles problem (which is a special case of our problem with $d=2$) by Mitchell [FOCS'21] and G\'{a}lvez, Khan, Mari, M\"{o}mke, Reddy, and Wiese [SODA'22].

==> PartitionSoCG.tex <==
\subsection{The partitioning lemma}
\label{sec:partitioning1}



We say that a curve $\gamma$ of the plane is \emph{monotone} if the intersection of $\gamma$ with any vertical line is a connected set. \fabr{Is "connected" defined? Maybe convex is equivalent here}

\begin{definition}[$t$-fence]
\label{def:fence}
    Let $t\ge 0$ be an integer. We say that a curve $\gamma$ of the plane is a $t$-fence if (i) $\gamma$ is the union\fabr{I think it is better to say "polygonal chain with $t$ segments"} of at most $t$ line segments, (ii) $\gamma$ is monotone, (iii) $\gamma$ is embedded in the grid $\calg$, (iv) $\gamma$ does not intersect any polygon in $\OPT$. 
\end{definition}
\anote{do fences need to start at non-degenerate edges? if yes, this could lead to quite many problems}


Let $C$ be a container. Let $P\in\OPT(C)$. 
A left side (right side) of $C$ is a vertical edge of $C$ that has $C$ on its right (left, respectively). Similarly, we say the $e_1(P)$ ($e_{d+1}(P)$) is the right edge (left edge, respectively) of a polygon $P\in \cP$, and for ease of readability, we denote $r(P):= e_1(P)$ and $l(P):=e_{d+1}(P)$. 

\begin{definition}[Structured container]
   \label{def:structured_container}
   [definition to be smoothed later]
    A container $C$ is\fabr{Here I'm lost: the boundary of a container contains fences? Where did we define containers this way?}\mnote{I agree that this is confusing, maybe we should call those differently?} said to be structured if its boundary can be ordered in a counter-clockwise fashion as a sequence $(s_1,\gamma_1, s_2,\gamma_2, \dots, s_\kappa,\gamma_\kappa)$ such that:
\begin{enumerate}[label=(\roman*)]
    \item for all $i\in [\kappa]$, $s_i$ is a vertical edge contained in the grid $\calg$, and $\gamma_i$ is a $(d-1)$-fence that not contain any vertical edges,
     \anote{the definition of fence becomes a bit circular here, a fence is already defined to be in $C$ above...}
     \item there exists an index $\kappa'$, with $1\le \kappa'\le \kappa-1$, such that for all indices $i$, with $1\le i\le \kappa'$, $s_i$ is a left edge of $C$ and for all indices $i$, with $\kappa'+1\le i\le \kappa$, $s_i$ is a right edge of $C$, and      
     %for any indices $i_1, i_2, i_3, i_4$ such that $1\le i_1 < i_2 < i_3 < i_4 \le \kappa$, if $e_{i_1}$ and $e_{i_3}$ are both left edge of $P$ (or both right edges of $P$), then either $e_{i_2}$ or $e_{i_4}$ is also a left edge (a right edge, respectively). 
     \item $2\le \kappa\le 10$.
\end{enumerate} 
\end{definition}

%back-up:
%\begin{definition}[Structured container]
%   \label{def:structured_container}
%    A container $C$ is\fabr{Here I'm lost: the boundary of a container contains fences? Where did we define containers this way?}\mnote{I agree that this is confusing, maybe we should call those differently?} said to be structured if its boundary can be ordered in a counter-clockwise fashion as a sequence $(s_1,\gamma_1, s_2,\gamma_2, \dots, s_\kappa,\gamma_\kappa)$ such that:
%\begin{enumerate}[label=(\roman*)]
%    \item for all $i\in [\kappa]$, $e_i$\fabr{Maybe $e_i\to s_i$} is a vertical edge contained in the grid $\calg$, and $\gamma_i$ is a $2d$-fence,
%     \anote{the definition of fence becomes a bit circular here, a fence is already defined to be in $C$ above...}
%     \item there exists an index $\kappa'$, with $1\le \kappa'\le \kappa-1$, such that for all indices $i$, with $1\le i\le \kappa'$, $s_i$ is a left edge of $C$ and for all indices $i$, with $\kappa'+1\le i\le \kappa'$, $s_i$ is a right edge of $C$, and      
     %for any indices $i_1, i_2, i_3, i_4$ such that $1\le i_1 < i_2 < i_3 < i_4 \le \kappa$, if $e_{i_1}$ and $e_{i_3}$ are both left edge of $P$ (or both right edges of $P$), then either $e_{i_2}$ or $e_{i_4}$ is also a left edge (a right edge, respectively). 
%     \item $2\le \kappa\le 5$.
%\end{enumerate} 
%\end{definition}




Notice that this definition allows some $\gamma_i$ to contain vertical edges. However, since such vertical sides are part of a fence, they do not intersect any polygon in $\OPT$. Also, it follows from this definition and by the definition of fences, that a structured container has at most $5(2d+1)=O(d)$ edges.  

\begin{definition}[Protected polygon]
\label{def:protected_polygon}
Let $C$\fabr{Very hard to parse! A figure?}  be a structured container, and let $P\in\OPT(C)$. %, and let $\calb=(s_1,\gamma_1, s_2,\gamma_2, \dots, s_\kappa,\gamma_\kappa)$ be a partition of its boundary that satisfies all conditions of Definition \ref{def:structured_container}. 
\begin{itemize}
    \item We say that $P$ is \emph{protected in $C$ from the left} if the left edge of $P$ intersects a left edge of $C$'s boundary or if there exists a polygon $P'\in\OPT$ that sees $P$ and that is intersected by the boundary of $C$. 
    \item We say that $P$ is \emph{protected in $C$ from the right} the right edge of $P$ intersects a right edge of $C$'s boundary or if $P$ is chargeable but does not see any polygon $P'\in\OPT(C)$. 
\end{itemize}
We say that $P$ is \emph{protected} in $C$ if it is either protected from the left or from the right. 
 \end{definition}\mnote{I believe this should be the best definition, for several reasons}

%Let $f$ be a $2d$-fence. We say that $f$ is a left fence (right fence), with respect to $C$ and $\calb$, if $f$ is contained in $C$ and if its left endpoint (right endpoint, respectively) is contained in a left edge (right edge, respectively) $s_i$ of $C$ for some $i\in[\kappa]$. 

%We say that a polygon $P\in \OPT(C)$ is protected (with respect to $C$ and $\calb$) from the left (from the right) if there exist two left fences (two right fences, respectively) $f_b$ and $f_t$ such that:
%\begin{enumerate}[label=(\roman*)]
%    \item $f_t$'s left endpoint (\fab{right} endpoint, respectively) and $f_b$'s left endpoint
%(\fab{right} endpoint, respectively) are both contained in the same left edge (right edge, respectively) of $C$,
%    \item $f_t$'s right endpoint (left endpoint, respectively) and $f_b$'s right endpoint
%(left endpoint, respectively) are both contained in $r(P)$ ($l(P)$, respectively), and \enote{are both contained in $l(P)$ ($r(P)$, respectively) ?}
%    \item edges\enote{edges? or segments? \fab{The pieces of a fence should be called segments, ok good suggestion!}} of $f_b$ and $f_t$ are disjoint, and
%    \item $f_b$ is below\fabr{Below/above defined? not really I agree} $P$ and $f_t$ is above $P$. 
%\end{enumerate}
%\end{definition}



% back-up: previous definition
%\begin{definition}[Left/right fence, protected polygon]
%\label{def:protected_polygon}
%Let $C$ be a structured container, and let $\calb=(s_1,\gamma_1, s_2,\gamma_2, \dots, s_\kappa,\gamma_\kappa)$ be a partition of its boundary that satisfies all conditions of Definition \ref{def:structured_container}. Let $f$ be a $2d$-fence. We say that $f$ is a left fence (right fence), with respect to $C$ and $\calb$, if $f$ is contained in $C$ and if its left endpoint (right endpoint, respectively) is contained in a left edge (right edge, respectively) $s_i$ of $C$ for some $i\in[\kappa]$. 
%
%We say that a polygon $P\in \OPT(C)$ is protected (with respect to $C$ and $\calb$) from the left (from the right) if there exist two left fences (two right fences, respectively) $f_b$ and $f_t$ such that:
%\begin{enumerate}[label=(\roman*)]
%    \item $f_t$'s left endpoint (left endpoint, respectively) and $f_b$'s left endpoint
%(left endpoint, respectively) are both contained in the same left edge (right edge, respectively) of $C$,
%    \item $f_t$'s right endpoint (left endpoint, respectively) and $f_b$'s right endpoint
%(left endpoint, respectively) are both contained in $r(P)$ ($l(P)$, respectively), and \enote{are both contained in $l(P)$ ($r(P)$, respectively) ?}
%    \item edges\enote{edges? or segments?} of $f_b$ and $f_t$ are disjoint, and
%    \item $f_b$ is below $P$ and $f_t$ is above $P$. 
%\end{enumerate}
%\end{definition}





%Notice that since $\gamma_i$'s endpoints are respectively contained in $s_i$ and in $s_{(i+1 \mod \kappa)}$, $\gamma_i$ is either a left \fab{or} a right fence (with respect to $C$ and $\calb$). 

%Let $C$ be a container. We say that $P\in \OPT(C)$ is protected from the left (protected from the right) (with respect to $C$) if there exists a left $d$-fence $f$ of $C$ (right $d$-fence of $C$) such that its right endpoint (left endpoint, resp.) is contained in a left edge (right edge, resp.) of $P$. In this case, we say that $P$ is protected by $f$.  
%If $P$ is either protected from the left or protected from the right, we say that $P$ is protected in $C$. 

%\begin{claim}
   % If $P$ is protected in $C$, then any side $e$ of $P$ is contained in a left (or right) $2d$-fence of $C$.
%\end{claim}
%
%\begin{proof}
%    Indeed, suppose that $P$ is protected from the left (the case when $P$ is protected from the right is similar). There exists a left $d$-fence $f$ of $C$ whose right endpoint $p$ is on $l(P)$. Suppose that $e$ has direction $v_i$, with $i\in [d]$ (resp. with $i\in\{d+1,\dots, 2d\}$). Let $\gamma$ be the portion of the $P$'s boundary from $e$ to $p$ following $P$'s boundary counter-clockwise (resp. clockwise). 
%    Let $f':= f\cup \gamma\cup e$.
%    Then $f'$ is a left $2d$-fence of $C$ since there are at most $d$ line segments in $\gamma\cup e$.
%\end{proof}  

%Let $C$ be a container. We say that a $t$-fence $\gamma$ is a left $t$-fence of $C$ (right $t$-fence of $C$) if (i) $\gamma$ is contained in $C$, (ii) the left endpoint (right endpoint, respectively) of $\gamma$ is contained in a left edge (right edge, respectively) of $C$, and (iii) $\gamma$ does not intersect any polygon $P\in\OPT(C)$.  \enote{We can assume that area $A(\gamma)$ specified by a fence is convex, and that  $A(\gamma)$ does not intersect any $P\in\OPT(C)$.}



\partitioning*


\subsection{Analysis via charging}
\label{sec:analysis}
In this section we show Lemma~\ref{lem:existenceRecursivePartition}, i.e., we show that for the set $\calp'$ constructed in Section~\ref{sec:construction} it holds $|\calp'|\ge |Z| + \frac{1}{2} |\calp|$.
In the construction of the recursive partition, the only reason why a polygon $P\in \OPT$  might be ``lost'' is that it is intersected by the boundary of some $C_u$ for $u\in T$. 
Lemma~\ref{lem:recursivePartitionContainsZ} states that this can happen only in the case~\ref{step:partition}.
Our goal is to show that we can ``lose'' at most half of $\calp$.

First, we describe in more detail the construction of the recursive partition for the internal nodes of $T$ in the case~\ref{step:partition}.
Let $u$ be an internal node of $T$, i.e., a node $u$ with  $|\OPT(C_u)|\ge 2$.
Recall that our tree $T$ has two nodes $u_1$ and $u_2$ corresponding to the structured containers $C_1$ and $C_2$, respectively.
The partition $\{C_1, C_2\}$ of $C_u$ is given by \fab{the} Partitioning Lemma. 

By \fab{the} Partitioning Lemma~\ref{verticalLine} it is clear that $\OPT(C_u) \setminus \{\OPT(C_1)\cup \OPT(C_2)\}$ is exactly the set of polygons in $\OPT(C_u)$ that are intersected by the vertical line segment $\ell_u$.
Our goal is to show that at most half of the polygons in the set $\calp$ are intersected by a vertical line segment for some node of $T$.

We will define a \emph{charging scheme} for the polygons in $\calp$ that are intersected by the vertical line $\ell_u$. 
For every node $u \in T$, and every polygon $P \in \OPT(C_u) \cap \calp$ that is intersected by the vertical line $\ell_{u}$ we charge $1$ to any polygon in $\OPT(C_u)$ that $P$ sees. 

By the definition of $\calp$, there exists a polygon $P'\in \OPT$ such that $P$ sees $P'$; but we need to show that such a polygon also exists in $\OPT(C_u)$ at the moment when $P$ is intersected by the vertical line segment $
\ell_u$. Intuitively, the reason is that if such a $P'$ does not exist, then $P$ must be protected by a fence from the right, which would contradict Partitioning Lemma~\ref{protectedSafe}.

We then need to ensure that in the overall process each polygon is charged at most once. 
Further more, if a polygon is charged then it will be protected (by the fences) for the rest of the partitioning process. 
Intuitively, the reason is that when $P'$ is charged due to a vertical line $\ell_u$, 
then it will be protected by a fence from the left. 

\begin{lemma}\label{lem:fencesFromRight}
    Let $P\in \calp$ be a polygon that is intersected by the vertical line segment $\ell_u$ for an internal node $u\in T$.
    Let $P'\in \OPT$ be a polygon seen by $P$.
    Then $P'\in \OPT(C_u)$.
\end{lemma}
\begin{proof}
    For the sake of contradiction, suppose that $P' \not \in \OPT(C_u)$. 
    Let $u'$ be the inner node of $T$ where the polygon $P'$ was intersected by the vertical line $\ell_{u'}$.
    Clearly, $u'$ is an ancestor of $u$ as otherwise $P' \in \OPT (C_{u'})$.

    Let $C_1$ be the child of $C_{u'}$ containing $P$. We claim that $P$ is protected in  $C_1$.
    By definition of $P$ seeing $P'$ we have that $t(e_{d+1}(P'))$ is contained in $\interior(e_1(P'))\cup \{b({e_1(P')})\}$.
    Let $p_t$ be upper and $p_b$ bottom of the two intersection points of $\ell_{u'}$ and the boundary of $P'$. See Figure~\ref{fig:lemma23}.
    Then, consider the curves $\gamma_t, \gamma_b$ that start in $p_t$ and $p_b$ respectively, then follow the boundary of $P$ until they reach $t(e_{d+1}(P'))$. 
    Clearly, each of the $\gamma_t, \gamma_u$ is a union of at most $d$ segments, and both of $\gamma_t, \gamma_u$ are monotone. 
    Since, $t(e_{d+1}(P'))$ is contained in $\interior(e_1(P'))\cup \{b({e_1(P')})\}$ it follows that $\gamma_t$ and $\gamma_b$ are  right $d$-fence for $P$ in $C_1$.  
    Thus,  $P$ is protected (from the right) in $C_1$.
    As $u$ is an successor of $u'$, and the partitioning never cuts the fences, it follows that $P$ is protected in $C_u$.
    This is a contradiction since the vertical line segment $\ell_{u}$ cannot intersect a protected polygon.
\end{proof}
\begin{figure}%
\centering
\includegraphics[width=0.4\textwidth]{lemma23.eps}%
\caption{Illustration for the proof of Lemma~\ref{lem:fencesFromRight}.}%
\label{fig:lemma23}%
\end{figure}

\begin{lemma}
    If a polygon $P'\in \OPT$ is charged, then $P' \in \calp'$, i.e., for a leaf $q$ of $T$ we have $\OPT(C_q) = P'$. 
    Moreover, $P'$ can be charged at most once.
\end{lemma}
\begin{proof}
    Each polygon $P'$ is charged at most once since there is at most one other polygon $P\in \OPT$ such that $P$ sees $P'$ Lemma~\ref{lem:chargingIsInjective}.

    Suppose $P'$ is charged by a polygon $P$ during the partitioning of $C_u$ for $u\in T$.
    In particular, $P$ sees $P'$ and thus $t(e_{d+1}(P'))$ is contained in $\interior(e_1(P'))\cup \{b({e_1(P')})\}$.
    Let $p_t$ be one the top and $p_b$ the bottom of the two intersection points of $\ell_u$ and the boundary of $P$.
    Then, consider the curves $\gamma_t, \gamma_u$ that start in $p_t, p_b$ respectively, follow the boundary of $P$ until they reach $t(e_{d+1}(P'))$. 
    Such curves $\gamma_t, \gamma_b$ exist since $P$ sees $P'$, and for the same reason we conclude that each of them is a union of at most $d$ segments, and that these curves are  is monotone.  
    Thus, in any container $C_i$ with $\ell_u$ as a part of its boundary, we have that $P'$ is protected (from the left) as $\gamma_t, \gamma_b$ are left $d$-fences.
    Hence, $P'$ is protected in the child node of $u$ that contains it.
    As we only ever intersect the polygons in $\OPT$ by a vertical line, and these never intersect the fences the polygons $P'$ remains protected in all the successors as well.
    This proves the lemma.
\end{proof}

\mainLemma*

\begin{proof}
By Lemma~\ref{lem:TisRecursive} we have that $T$ is a recursive partition for $\calp'$. 
By Lemma~\ref{lem:exists_good_option}, 
we have that $\calp \ge \frac{3}{4d} |\OPT\setminus Z|$.
By Corollary~\ref{cor:recursivePartitionContainsZ}, $Z\subseteq \calp'$.
Then, since $Z\cap \calp = \emptyset$ and by the charging described above, we have $|\calp'| \ge |Z| + \frac{1}{2} |\calp|$ as for each polygon $P\in \calp$ that is lost during the partitioning in the recursion, we keep in $\calp'$ one of the polygons that $P$ sees. 
The lemma follows since $|\calp| \ge \frac{3}{4d} |\OPT\setminus Z|$.
\end{proof}


\subsection{Proof of the partitioning Lemma}
\label{sec:paritioning2}
\mnote{some figures would be very helpful here \fab{I would say necessary: section 4 is very hard to read!}}

\partitioning*
We will prove the following stronger version of the Partitioning Lemma. 
\enote{We state the weaker version in S2 that contains the minimum needed for understanding the bigger picture. Here we actually state the strongest version that is easier to prove.}
\begin{lemma}
\label{lem:paritioningStronger}
    Let $C$ be a structured container (with $k=O(d)$ sides), and such that $|\OPT(C)|\ge 2$.  
    
    Then, there exists a set $\Gamma$ of line segments, such that
    \begin{enumerate}[label=(\Alph*)]
        \item $\Gamma$ is composed of at most $4d+1$ line segments that are all contained in $C$, and embedded on the grid $\calg$. 
        \item $\Gamma$ partitions $C$ into two structured containers $C_1$ and $C_2$, that are both strict subsets of $C$.         \item\label{verticalLine} There exists a vertical line segment $\ell\in \Gamma$ that intersects all the polygons in $\OPT(C)$ that are intersected by $\Gamma$.
        \item\label{protectedSafe} $\Gamma$ does not intersect any polygon of $\OPT(C)$ that are protected in $C$. 
    \end{enumerate}    
\end{lemma}

[todo: case when $C$ has only few edges. ]

Let $C$ be a structured container, and let $\calb=(s_1,\gamma_1, s_2,\gamma_2, \dots, s_\kappa,\gamma_\kappa)$ be the sequence of curves that form the boundary of $C$ as in Definition \ref{def:structured_container}. %We assume without loss of generality that $e_1$ is a left edge and $e_\kappa$ is a right edge. 
%Let $s\in[\kappa]$ be the index such that $e_s$ is a left edge and $e_{s+1}$ is a right edge. By the definition, we know that $C$ has $s$ left edges that are $e_1, e_2, \dots, e_r$ and $\kappa-s$ right edges that are $e_{\kappa+1}, e_{\kappa+2}, \dots, e_\kappa$. 

The proof is in two parts. We first treat the case where $2\le \kappa\le 4$, and then we treat the case when $\kappa=5$. 

\paragraph{$2\le\kappa\le 4$.} TODO

\paragraph{$\kappa=5$.} 

We recall that there is an index $\kappa'$ with $1\le \kappa'\le 4$, such that all edges $s_1,\dots,s_{\kappa'}$ are left edges and all edges $s_{\kappa'+1},\dots,s_5$ are right edges. 
Without loss of generality, we assume that $\kappa'\ge 3$. For otherwise, apply a vertical symmetry to $C$ and apply the following strategy on the mirror of $C$. 



We construct $\Gamma$ and then show that $\Gamma$ satisfies the desired conditions. To construct we first need the notion of witness of a protected polygon. 

 Let $P\in\OPT(C)$ be a polygon protected in $C$. Suppose first that $P$ is protected  from the left. Suppose first that the left edge of $P$ intersects a left vertical edge $s_i$ of $C$, for some index $i\le \kappa'$. Then we say that $s_i$ is the witness of $P$. (Notice that in the case where the left edge of $P$ intersects several left vertical edges of $C$, then we can create a cut $\Gamma$, that connects such two vertical edges; and it is easy to check that $\Gamma$ satisfy all conditions of Lemma \ref{lem:paritioningStronger}.) Otherwise, $P$ is protected from the left in $C$ because there exists a polygon $P'\in \OPT$ such that $P'$ sees $P$, and that is intersected by the boundary of $C$. Since by definition, fences do not intersect any polygon in $\OPT$, there exists an index $i\in [\kappa]$, such that $P'$ is intersected by $s_i$. By construction of a structured polygon, it is easy to see that there such an edge is unique and is a left edge, i.e., $i\le \kappa'$. We call $s_i$ the \emph{witness} of $P$. 

 Now suppose that $P$ is protected from the right. First, assume that the right edge $r(P)$ of $P$ is contained $s_i$, for some index $i\in [\kappa]$. In this case, we say that $s_i$ is the witness of $P$. (As before, we can assume without loss of generality that the right edge of $P$ does not intersect several vertical edges of $C$.). % in the bounding box $C^*$. Then, since $P\subseteq C\subseteq C^*$, there exists a right edge $s_i$ of $C$, for some $i$ with $\kappa'+1\le i \le 5$, such that $r(P)$ is contained in $s_i$. In this case, $s_i$ is the witness of $P$. 
 Otherwise, $P$ sees a polygon $P'\in\OPT$ that is not in $\OPT(C)$. The right edge of $P$ and the left edge of $P'$ intersect. Thus, since $P\subset C$ and $P'\not\subset C$, we deduce that $C$'s boundary intersects the boundary of $P'$. If $C$'s boundary intersects $P'$, then there exists a unique right edge $s_i$ of $C$ that intersect $P'$. In this case, we say that $s_i$ is the witness of $P$. Otherwise, that is when  
or $C$'s boundary and the boundary of $P'$ intersect, but $C$'s boundary does not intersect $P'$, it must be that there exists a right vertical edge $s_i$ of $C$, for some index $i\in[\kappa]$, that intersects both $l(P')$ and $r(P)$. In this case, we say that $s_i$ is the witness of $P$. 

Notice that the witness of a polygon protected from the left (from the right) is a left edge of $C$ (right edge of $C$, respectively). %In the latter case, it is easy to see that $C$'s boundary only intersect 
% It is easy to see that if $P'$ is not intersected by the boundary of $C$, i.e., if $P'$ is completely outside $Thus, $P$
 
 %We first define the witness of a polygon protected in $C$ as follows. Let $P$ be an

Now we partition the set of left edges into three groups: the top ones $E_T:=\{s_1,\dots,s_{\lfloor \kappa'/3\rfloor}\}$, the middle ones $E_M:=\{s_{\lfloor \kappa'/3\rfloor+1},\dots,s_{\lfloor 2\kappa'/3\rfloor}\}$, and the bottom ones $E_B:=\{s_{\lfloor 2\kappa'/3\rfloor+1}, \dots,{s_{\kappa'}}\}$. 

Let $p$ be the rightmost point in $C$ such that $p$ is on the right edge of a polygon $P_0\in\OPT(C)$ that is protected from the left and has a witness in the middle group $E_M$. % by two left fences $f_b$ and $f_t$ whose left endpoints are contained in $s_2$. %some left edge $e\in E_M$, i.e., from the middle group. 
In the case of ties, we pick an arbitrary one. %In particular, there exists a left $2d$-fence $f$ of $C$ whose right endpoint is $p$ and whose left endpoint is on a left edge of $C$ that is contained in $E_M$.  %with the rightmost right endpoint among all left $2d$-fences of $C$ whose left endpoint is contained in some left edge of the middle group $E_M$.  Let $p$ denote the right endpoint of $f$. 

Now, let $p_t$ and $p_b$ the two points that satisfy the following conditions: 
\begin{enumerate}
    \item[(i)] $p_t$ and $p_b$ are in the same vertical line as $p$, $p_t$ is above or coincides with $p$ and $p_b$ is below or coincides with $p$.
    \item[(ii)] $p_t$ ($p_b$) is either contained in the boundary of $C$ or, $p_t$ ($p_b$, resp.) is contained in the boundary of some polygon $P_t\in\OPT(C)$ ($P_b\in\OPT(C)$, respectively), that is protected and such that $p_t$ ($p_b$, resp.) is neither contained in the left nor the right edge of $P$. 
     \item[(iii)] The semi-open vertical line segments $[p,p_t[$ and $[p,p_b[$ do not contain any point that satisfies condition (ii). 
\end{enumerate}
It is clear that these two points exist and are unique. 

[description of $\gamma'$]

It follows from condition (ii) and from Definition \ref{def:protected_polygon} that $p_t$ is contained in a left (or right) fence $\gamma'_t$ of $C$. Indeed, $\gamma'_t$ either corresponds to the left (or right) fence that protects $P$ from below (i.e., $f_b$ in Definition \ref{def:protected_polygon}), or $\gamma'_t$ corresponds to some $\gamma_i$, from some $i\in [\kappa]$. Without loss of generality, we assume that $p_t$ is the right (left, respectively) endpoint of $\gamma'_t$. Similarly, there exists a left (or right) fence $\gamma'_b$ whose right (left, respectively) endpoint is $p_b$. We now define $\Gamma$ depending on which of the following cases we are.
\begin{description}
    \item[(case a)] If $\gamma'_t$ is a right fence, then define $\gamma'_1=f_t$, $\gamma'_2:=\gamma'_t$ and $\ell = [p,p_t]$.
    %$\Gamma':=f\cup \ell\cup f_t$, where  
    \item[(case a')] Otherwise if $\gamma'_b$ is a right fence, then define $\gamma'_1=f_b$, $\gamma'_2:=\gamma'_b$ and $\ell = [p,p_b]$.
    %$\Gamma':=f\cup \ell\cup f_b$, where $\ell = [p,p_b]$. 
    \item[(case b)] Otherwise, both $\gamma'_t$ and $\gamma'_b$ are left fences of $C$. Then, define $\gamma'_1=\gamma'_t$, $\gamma'_2:=\gamma'_b$ and $\ell = [p_t,p_b]$.
    %Then define $\Gamma':=f_t\cup \ell\cup f_b$, where $\ell=[p_t,p_b]$. 
\end{description}
    
We now define $\Gamma':= \gamma'_1\cup \ell\cup \gamma'_2$. % depending on which of the following cases we are.
%Let $\ell$ be the longest vertical line segment that (i) contains $p$, (ii) is contained in $C$, and (iii) does not intersect any polygon protected in $C$. Let $t$ denote the top endpoint of $\ell$ and let $b$ denote its bottom endpoint. By the definition of $\ell$, $t$ and $b$ are both either contained in the boundary of a polygon protected in $C$ or contained in the boundary of $C$. [to continue]

%that the interior of $\ell$ is disjoint from the boundary of $C$. 
%We now define $\Gamma$ as the connected largest subset of 

[todo: deal with degenerate cases, where $\Gamma'$ intersects several times the boundary. I guess we want to define a $\Gamma$ whose interior is strictly inside $C$]. 

\anote{A big problem that could arise is if fences \emph{intersect}: we could get a lot of connected components}

We now show that $\Gamma$ satisfies each of the conditions of Lemma \ref{lem:paritioning}. 
\begin{enumerate}[label=(\Alph*)]
    \item By construction, $\gamma$ is a subset of the union of two $2d$-fences --- which, by definition, are embedded in the grid $\calg$ --- and the vertical line segment $\ell$. Since $\ell$ contains a point, $p$, that is contained in the right edge of an input polygon, $\ell$ is contained in the grid. Thus, $\Gamma$ is contained in $\calg$. Furthermore, $\gamma$ contains at most $4d+1$ line segments. 
    \item %f [todo: construct the edge sequence, and then argue that $\kappa\le 13$]
    We first construct $C_1$ and $C_2$, and then argue the desired properties. 
    Let $s_{i_1}\in \{s_1,s_2\}$ and $s_{i_2}\in \{s_3,s_4,s_5\}$ respectively denote the vertical edges of $C$ on which fences $\gamma'_1$ and $\gamma'_2$ are anchored. %For all $e'\in \{e,e_t,e_b\}$, we define $i(e')$ as follows. If $e_1=s_i$ for some index $i\in [\kappa]$, then define $i_1:=i$; otherwise, there exists an index $i\in [\kappa]$ such that $e_1\in \gamma_i$, and in this case define $i_1:=i$. We define $i_2$ in the same way. 
  We claim that $2\le i_2-i_1\le 4$. Indeed, in (case a) and (case a'), we have $i_1=2$ and $ 4\le i_2\le 5$, and in case %, which implies that $\kappa'/3\le i_2-i_1\ge \kappa-\kappa'/3$. In 
  (case b), we have $i_1=1$ and $3\le i_2\le 4$. %, which implies $\kappa'/3\le i_2-i_1\ge \kappa'-1\le \kappa/2-1$
    We construct the boundaries $\calb_1$ and $\calb_2$ of the components $C_1$ and $C_2$ as follows. Let $q_1$ denote the endpoint of $\gamma'_1$ that is on $s_{i_1}$. $s_{i_1}\setminus q_1$ consists in two vertical segments (one of those may possibly be empty): $s^1_{i_1}$ that is above $q_1$ and $s^2_{i_1}$ that is below $q_1$.  Similarly, we partition $s_{i_2}:=s^1_{i_2}\cup s^2_{i_2}$. Now, we define 
    $\calb_1=(s_1,\gamma_1,\dots, s^1_{i_1},\gamma'_1,\ell,\gamma'_2,s^1_{i_2},\gamma_{i_2},\dots, s_5,\gamma_5)$; 
    and $\calb_2=(s^2_{i_1},\gamma_{i_1},s_{i_1+1},\gamma_{i_1+1},\dots, s^2_{i_2},\gamma'_2,\ell,\gamma'_1)$. 
    In (case a), it turns out that $\ell$ is a left edge of $C_2$. In this case, we re-index the elements of $\calb_2$, so that the first left edge of $\calb_2$ is now $\ell$. 
    It is clear that $C_1$$C_1\cup C_2$
    It is not difficult to check that $(C_1,\calb_1)$ and $(C_2,\calb_2)$ are both satisfy all conditions of Definition \ref{def:structured_container}, thus $C_1$ and $C_2$ are structured containers. 
    \item By definition, fences of $C$ do not intersect any polygon in $OPT(C)$, thus if some polygon in $OPT(C)$ is intersected by $\Gamma$, it has to be intersected by the vertical line segment $\ell$.
    \item Suppose for the sake of a contradiction that $\Gamma$ intersects a polygon $P\in \OPT(C)$ that is protected in $C$. By the previous point, we know that $P\cap \Gamma\subset \ell$. Suppose for now that $\ell$ intersected twice the boundary of $P$. Let $q_t$ and $q_b$ denote the top intersection point and the bottom intersection point of $\ell$ with the boundary of $P$. If $p\in [q_b,q_t]$, then by convexity of $P$, we deduce that $p$ is in the interior of $P$. But $p$ is on the right edge of another polygon, which brings a contradiction with the assumption that polygons in $\OPT$ do not intersect. Thus, either $q_b$ is above $p$, or $q_t$ is below $p$. We treat the case when $q_b$ is above $p$, and the other case is obtained symmetrically. We obtain a contradiction we the definition of $p_t$. Indeed, we know that $q_b\in [p,p_t[$, and we by assumption, $q_b$ satisfies condition (ii). Thus, $\Gamma$ does not intersect any polygon that is protected.  
    %\item ??? \mat{Why do we need this?} \edi{Maybe we don't. I just wanted a reference for the claim "Once the polygon is protected, it remains protected until the end of recursive partition."; but this should just be moved to the proof of Lemma 24.}
    %\item Let $P\in \OPT(P)$ be a polygon intersected by $\ell$ and assume that $P$ is chargeable. Then, there exists a polygon $P'\in\OPT$ such that the right edge of $P$ and the left edge of $P'$ intersect. Suppose for the sake of a contradiction that $P'\notin \OPT(C)$. \mat{[TODO: it seems to be the same as claim 23]}
\end{enumerate} 

==> notation_list.tex <==
\subsection{Notation and terminology}
\label{sec:notation}
\enote{Not up to date, we are thinking of defining the notation only in the sections where we use it.}
\begin{itemize}
    \item \emph{Direction defining vectors} $\cald = \{v_1, \dots, v_{d}\} \subseteq \Z_{+} \times \Z$. W.l.o.g.\ assume $v_1 = (0,1)$, $v_2^2/v_2^1 < v_3^2/v_3^1 < \dots < v_{d}^2/v_{d}^1$, i.e. $v_i$'s are ordered in increasing slope. For $i \in \{d+1, \dots, 2d\}$, let $v_i \coloneqq -v_{i-d}$.
    \item Convention: Write vector component indices as exponent. For vector $w=(w^1, w^2) \in \R^2$, define $w^\perp \coloneqq (w^2, -w^1)$ (clockwise orthogonal rotation).
    \item $[k] = \{1, \dots, k\}$.
    \item Polygon $P = \angl{p_1, \dots, p_{2d}} \coloneqq \{x\in \R^2:\ x^\intercal v^{\perp}_i < p_i,\ \forall i \in [2d]\}$. We assume that all constraints (also redundant ones) are tight, i.e.\ $P \cap \{x:\ x^\intercal v^{\perp}_i = p_i\} \neq \emptyset$ for every $i \in [2d]$.
    \item Set of all polygons is $\cali$, $n = |\cali|$.
    \item Two polygons intersect/conflict/overlap if and only if their interiors intersect. In particular, two polygons do not intersect if they overlap only at corners or edges.
    \item Edge $e_i(P) \coloneqq P \cap \{x:\ x^\intercal v^{\perp}_i = p_i\}$. 
    %\setminus \{x:\ x^\intercal v^{\perp}_{i+1} = p_{i+1}\}$. 
    Edge $e$ of of $P$ is called a \emph{degenerate edge} if $e = \emptyset$.\fabr{Empty set or it is a single point?}
    Notice that the line segments $e_1(P), \dots, e_{2d}(P)$ form a positively/counter-clockwise oriented Jordan-curve. Moreover, by the definition of $v_i$ for $i \in \{d+1, \ldots, 2d\}$ the edges $e_i$ and $e_{d-i}$ are parallel whenever they are non-degenerate. 
    \item The bottom/starting point of the edge $e = e_i(P)$ of $P$ is $s(e) \coloneqq e_i(P) \cap \{x:\ x^\intercal v^*_{i-1} = p_{i-1}\}$. Similarly, the top/end point of $e = e_i(P)$ is $t(e) \coloneqq s(e_{i+1}(P))$.
    \item A $i$-directional Ray is a line of the form $v + \spn(v_i)$ (as a Minkowski sum). The $i$-directional ray intersecting the point $w$ is denoted as $\ray_i(w) \coloneqq w + \spn(v_i)$.
    \item Supporting grid $\calg$ is set of all rays spanned by the polygons in $\cali$
\end{itemize}

For indexes of directions, we think in modulo $2d$, e.g. $v_0 = v_{2d}$.


==> old_files/old_partitioning_lemma.tex <==
\subsection{Partitioning lemma}

\anote{I try to define a new concept of ``horizontal edge which could be helpful for building the partition lemma. it might also be }

\begin{definition}[Segment distance]
    Let $f$ be a curve along the directions $\cald$ with starting point $a$ and end point $b$ (which is possibly closed, i.e.\ $a=b$). The \emph{(horizontal) segment distance} between $a$ and $b$ over $f$, written $d_f(a,b)$, is defined as follows:
    \begin{itemize}
        \item If $f$ is a vertical line segment, then $d_f(a,b)=1$.
        \item If $C$ contains non-vertical line segments, $d_f(a,b)$ is defined as the number of vertical line segments (including virtual vertical edges)
        \anote{not sure about this}
        contained in $f$ plus the number of strictly $x$-monotonic segments of $f$.
    \end{itemize}
    The \emph{segment length $\ell(f)$ of $f$} is defined by $d_f(a,b)$.
\end{definition}

Notice that in particular, two non-equal points both lying on the top (resp.\ on the bottom) of a convex polygon have distance 1.

\begin{definition}
    Let $Q$ be simple (but not necessarily convex) polygon along $\cald$ and $q$ be a point on the boundary of $Q$. A \emph{curve fence emerging from $q$} is a strictly $x$-monotone curve with starting point $q$ lying inside $Q$. 
\end{definition}

\begin{remark}
    Notice that a fence always has length 1 and that w.l.o.g., we can assume that q lies on a vertical (possibly virtual) edge of $Q$.    
\end{remark}


\begin{definition}
    A simple (but not necessarily convex) polygon $Q$ is called \emph{horizontally quasi-convex} if any two points $a,b$ with identical $y$-value have segment distance 0 or 1 over some curve inside $Q$.
\end{definition}


For any polygon $Q$, let $\partial Q$ denote the border of $Q$.

\begin{lemma}[Partitioning Lemma]
    Let $Q$ be a horizontally quasi-convex simple polygon with circumference at most $k$
    %
    \footnote{the \emph{circumference} of a polygon is defined to be the length of its border with starting point being chosen to be at the top or bottom of a vertical line segment (which is well-defined). A convex polygon always has circumference 4.}
    %
    which contains at least two elements of $\OPT'$. Then there a set of curves $C$ such that
    \begin{enumerate}
        \item The curves in $C$ have cumulated length $k'$;
        \item $Q\setminus C$ has two or three components, each of them being horizontally quasi-convex and with circumference at most $k$;
        \item There exists a vertical line segment $t \in C$ such that all polygons in $\OPT'$ which are intersected by $C$ are intersected in $t$;
        \item $C$ does not intersect any protected polygon in $\calp$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    Let $T$ be the curve on 
\end{proof}



==> recursive_partition.tex <==

\section{Recursive partitioning}
\label{sec:recursivePartitioning}
Recall that $\OPT$ is a fixed optimal solution and that $\calp \subseteq \OPT$ is a set of chargeable polygons such that $|\calp| \ge \frac{3}{4d}|\OPT \setminus Z|$.
 
We will construct a recursive partition for a specific subset set $\calp' \subseteq \calp \cup Z$, such that $|\calp'| \ge|Z| + \frac{1}{2} |\calp|$.
This, proves Lemma~\ref{lem:existenceRecursivePartition}.

\subsection{The partitioning lemma}
\label{sec:partitioning1}

Consider a polygon $P$ with the counter-clockwise orientation of its boundary as before. 
Recall that we have already chosen a specific vertical-up direction. 
We this can used to consistently define
 \emph{top} of a polygon as the polygonal chain of line segments with directions $v_{2}, \dots, v_{d}$; and \emph{bottom} of a polygon as the polygonal chain of line segments with directions $v_{d+2}, \dots, v_{2d}$.  

\begin{definition}[Fence]\enote{They are not really fences as in the case of rectangles.}
\label{def:fence}
    Let $P_1 ,P_2 \in \OPT$ such that $P_1$ sees $P_2$. 
    Then there exists an edge segment $e' = [t(e_1(P_1)), h(e_{d+1}(P_2))$.%
    \footnote{
        Recall that $e_1(P)$ is the vertical-up edge of $P$ and $e_{d+1}(P)$ is the vertical-down edge of $P$.
    }
    
    A \emph{bb-fence} $(P_1, P_2)$ is a polygonal chain of line segments $\gamma$ obtained as a union of the bottom of a polygon $P_1$, the edge segment $e'$, and the bottom of a polygon $P_2$.
    Any continuous subset of this chain, is also called a bb-fence. 

    Similarly, we define a tt-fence. A polygonal chain of line segments $\gamma$ is a \emph{tt-fence} if it can be obtained as a union of a subset of the top of a polygon $P_2$, $e_{d+1}(P_2)\setminus e'$ and the top of $P_1$; or any continuous subset of this chain. 

    A \emph{fence} is either a bb-fence or a tt-fence. 
\end{definition}

Next, we specify a definition of a container. 

\begin{definition}[Structured container]
   \label{def:structured_container}
    A container $C$ is said to be \emph{structured} if its boundary consists of at most  $5$ cutting lines and at most $5$ fences such that 
    that the fences and the cutting lines alternate on the boundary of $C$.
    Moreover, left cutting lines are consecutive.
    \anote{how are left/right cutting lines defined? they have the interior of $C$ on their right/left?}
\end{definition}
It follows that a structured container has at most $5 + 5(2(d-1)+1) = 10d$ edges.  

\begin{definition}[Protected polygon]
\label{def:protected_polygon}
Let $C$\fabr{Very hard to parse! A figure?}  be a structured container, and let $P\in\OPT(C)$. 
We say that a polygon $P'\in \calp$ is \emph{protected in $C$ from the left via} $s$ if there exists a polygon $P\in\OPT$ that sees $P$ and that is intersected by a \edi{left?} cutting line $s$ of $C$. 
We say that a polygon $P\in \calp$ is \emph{protected in $C$ from the right via $s'$} there exists if $P'\in \OPT$ that is seen by $P$ and that is intersected by a \edi{right?} cutting line $s'$ of $C$.

We say that $P$ is \emph{protected} in $C$ if it is either protected from the left or from the right. 
\end{definition}

\partitioning*

\subsection{Construction of the recursive partition}
\label{sec:construction}
\enote{I am not sure what is the best order to put it in; the current one is not optimal as we start with construction, then partitioning lemma, analysis and then proof of the partitioning lemma. We could move 4.1 into 4.3 e.g. \fab{The partitioning lemma should be stated before, otherwise the rest is unreadable. The proof can be postponed} }

Let $C$ be a container. 
We define $\OPT(C)\subseteq \OPT$ the subset of polygons of $\OPT$ that are contained in $C$.

We construct a recursive partition $T$ for a subset $\cP'\subseteq \OPT$.
% such that $Z\subseteq \calp'$ and $|\calp'|\ge |Z| + \frac{1}{2} \calp$.
See Definition~\ref{def:recursivePartition}.
To construct the recursive partition $T$ and the set $\cP'$, we apply the following procedure. 
The root $r$ of $T$ corresponds to the bounding box $C^*$. 
Throughout the construction of $T$ we maintain a set of nodes $A$ for which the corresponding containers are yet to be partitioned, initialized with $A=\{r\}$. 
We also initialize $\cP'=\emptyset$. 

Our recursive procedure will first define the recursive partition  when the current container still contains a corner polygon. 
Once, we have processed all the corner polygons we will continue to recursively define the tree and partition $\calp'$ using the Partitioning Lemma. 
In particular, we will ensure that every node of $T$ corresponds to some special type of container, called a structured container, defined in the next subsection. 
 
%We also initialize $\cP'=\emptyset$. 
The construction of $T$ and $\cP'$ finishes when $A=\emptyset$. While there exists a node $u$ in $A$, we do the following:\fabr{Pseudocode (recursive) would be much more readable} 

\begin{enumerate}[label=(R\arabic*)]
    \item\label{step:Z} \textbf{Preprocessing $Z$.}
    Recall that $Z\subseteq \OPT$ is the set of corner polygons in $C^*$, i.e., polygons $P$ for which all but at most one edge of $P$ is contained in the boundary of $C^*$. (See Figure~\ref{fig:cornerPolygon}.)
    If $\OPT(C_u)$ contains a corner polygon say $P_z$, then we define $C_1 \coloneqq P_z$ and $C_2 \coloneqq (C_u \setminus P_z)\cup e$ for $e$ the unique edge of $P_z$ not contained in the boundary of $C^*$.
    These form \fab{a} partition of $C_u$. 
    Then, we create in $T$ two children of $u$ that we call $u_1$ and $u_2$. We set $C_{u_1}=C_1$ and $C_{u_2}=C_2$. 
    Finally, we add $u_1$ and $u_2$ to $A$ and remove $u$ from $A$.
    \item\label{step:emptyset} If $\OPT(C_u)=\emptyset$, we remove $u$ from $T$ and from $A$.
    \item\label{step:singleton}If $\OPT(C_u)=\{P\}$ for some $P\in \OPT$, then we set $P_u=P$, add $P$ in $\cP'$ and remove $u$ from $A$.
    \item\label{step:partition} \textbf{Partitioning $C_u$.} In\fabr{The split cannot create new corner polygons, right?} the remaining case we have $|\OPT(C_u)|\ge 2$ and $\OPT(C_u)$ contains no polygons from $Z$. 
    We apply the following partitioning Lemma~\ref{lem:paritioning} to $C_u$ stated below to obtain two containers $C_1$ and $C_2$ that form a partition of $C_u$. Then, we create in $T$ two children of $u$ that we call $u_1$ and $u_2$. We set $C_{u_1}=C_1$ and $C_{u_2}=C_2$.
    Finally, we add $u_1$ and $u_2$ to $A$ and remove $u$ from $A$.
\end{enumerate}

More detailed description of the case when $|\OPT(C_u)|\ge 2$ will be given in Section~\ref{sec:analysis} after we introduce the necessary notation and Partitioning Lemma in Section~\ref{sec:partitioning1}. 
In Section~\ref{sec:analysis}, we also show that $|\calp'| \ge |Z| + \frac{1}{2} |\calp| \ge \frac{3}{8d} |\OPT|$.

\begin{lemma}
\label{lem:TisRecursive}
    $T$ is a recursive-partition for $\cP'\subseteq \OPT$.  
    Moreover, every container obtained in~\ref{step:Z} is a convex polygon with at most $8$ line segments.
\end{lemma}
\begin{proof}
We need to prove each of the requirements for the recursive partition. 
We prove the first requirement, and we state the remaining ones for readability---these follow by construction.\fabr{Move the claims not relevant for the lemma as observations outside the proof}
    \begin{itemize}
        \item (Every node $u\in V$ corresponds to some container $C_u \in \calc$.) For the root this is the case since $C^*$ is a container. 
        Otherwise, $C_u$  for some $u\in$ is created in either~\ref{step:Z} or~\ref{step:partition}. Since $|Z|\le 4$ we are in the step~\ref{step:Z} at most $4$ times. See Figure~\ref{fig:cornerPolygon}. Moreover, these steps are the first four steps of our construction. 
        It is easy to check by definition of the corner polygons, that $C_1$ and $C_2$ have at most one segment more that $C_u$. 
        It follows that in a step~\ref{step:Z} we can only obtain polygons with at most $8$ sides; in particular these are containers. 
        In~\ref{step:partition}, \fab{the} Partitioning Lemma will guarantee that both $C_1$ and $C_2$ are containers (even more so, they are structured containers).
        \item (The root $r$ of $T$ corresponds to $C^*$, i.e. $C_r = C^*$.)
        \item (Every internal node has  $2$ children $u_1, u_2$ such that $C_{u_1}, C_{u_{2}}$ form a partition of $C_u$.) 
        \item (For every leaf $u$ of $T$, $C_u$ contains exactly one polygon $P_u \in \calp'$ or no polygon in $\calp'$.)
        \item (For every $P \in \calp'$, there exists a leaf $u$ of $T$ such that $P=P_u$.) \qedhere
    \end{itemize}
\end{proof}

\begin{lemma}\label{lem:recursivePartitionContainsZ}
    Let $u$ be an inner node of $T$ such that $C_u$ contains a corner polygon. Let $u_1$ and $u_2$ be the children nodes of $u$. 
    Then $\OPT(C_u) = \OPT(C_{u_1}) \cup \OPT(C_{u_2})$.
\end{lemma}
The lemma states,\fabr{We spend way too much time to handle $Z$ which is trivial: can't we just shave off $Z$ at the beginning in words and be formal only on the rest?} that the construction of the partition for the nodes $u$ where $C_u$ contains a polygon in $Z$ does not ``lose'' any of the polygons from $\OPT$ whenever we are in the case~\ref{step:Z}.
\begin{proof}[Proof of Lemma~\ref{lem:recursivePartitionContainsZ}]
Recall that $C_{u_1} = P_z$ for a corner polygon $P_z \in \OPT(C_u)$; and $C_{u_2} = (C_u \setminus P_z) \cup e$ where $e$ is the edge of $P_z$ not contained in the boundary of $C^*$.
In particular, this means that $C_u$ is partitioned along the edge $e$ into $C_{u_1}$ and $C_{u_2}$. 
In particular, $e$ does not intersect (the interior) of any polygon in $\OPT(C_u)$. The lemma follows.
\end{proof}

\begin{corollary}\label{cor:recursivePartitionContainsZ}
    The recursive partition $\calp'$ contains all the corner polygons, i.e.,  $Z\subseteq \calp'$.
\end{corollary} 

\begin{figure}%
\centering
\includegraphics[width=0.8\textwidth]{cornerPolygons.eps}%
\caption{Illustration of the corner polygons and the recursive partition in case~\ref{step:Z}.}%
\label{fig:cornerPolygon}%
\end{figure}

